Publicly Auditable MPC-as-a-Service with succinct verification and universal setup

In recent years, multiparty computation as a service (MPCaaS) has gained popularity as a way to build distributed privacy-preserving systems. We argue that for many such applications, we should also require that the MPC protocol is publicly auditable, meaning that anyone can check the given computation is carried out correctly -- even if the server nodes carrying out the computation are all corrupt. In a nutshell, the way to make an MPC protocol auditable is to combine an underlying MPC protocol with verifiable computing proof (in particular, a SNARK). Building a general-purpose MPCaaS from existing constructions would require us to perform a costly "trusted setup" every time we wish to run a new or modified application. To address this, we provide the first efficient construction for auditable MPC that has a one-time universal setup. Despite improving the trusted setup, we match the state-of-the-art in asymptotic performance: the server nodes incur a linear computation overhead and constant round communication overhead compared to the underlying MPC, and the audit size and verification are logarithmic in the application circuit size. We also provide an implementation and benchmarks that support our asymptotic analysis in example applications. Furthermore, compared with existing auditable MPC protocols, besides offering a universal setup our construction also has a 3x smaller proof, 3x faster verification time and comparable prover time.

==> constructions/subprotocols.tex <==
\section{Subprotocols:}
Here we list the sub protocols which we use for different operations in our construction
% \subsection{Polycommit scheme for shares of evaluations:}
% \label{sec:cli_commit_new}
% Our construction for Auditable MPC on Marlin relies on creating a Polynomial commitment to a polynomial from commitments off the shares of evaluations. Our key idea is that commit to a evaluation(share) of the polynomial by committing to a Lagrange polynomial multiplied by the share. We can later homomorphically combine the commitments to shares to obtain a commitment to the polynomial which we can we polyeval proofs. 
% We now define a new extractable trapdoor commitment scheme based on Lip'16 with three major adaptations.  
% \begin{itemize}
%     \item Lip'16 schemes uses evaluations of $\ell_i(\beta)$ for a trapdoor secret $\beta$. We instead use the standard $1, X, X^2$ and create a polynomial commitment
%     using Kate style polynomial commitments. Since, the our ZKsnark for Marlin is based on the that CRS, we use the same CRS as it allows us to use standard polycommit proof batching techniques for efficiency.
%     \item Lip'16 scheme was based on PKE assumptions and hence required double the elements in CRS and double the commitment size. Although it is possible to adapt out scheme to use that we rely on a weaker assumption, namely AGM for efficiency reasons.
%     \item We clearly highlight how to construct a polynomial commitment for giving evaluation proofs of polynomial which is shown in Lip'16.(Lip'16 was designed for Commit and prove snark and not as polycommit scheme, so it was not required for them to satisfy the evaluation proof properties).
% \end{itemize}
% Let $\mathbf{a} = (a_0, a_1, \ldots, a_{n-1})$ be a message vector of length $n$ which we wish to commit. Further, let For simplicity, we assume n is a power of two, and let
% \begin{itemize}
%     \item $\omega$ be the n-th primitive root of unity in a field $\mathbb{F}_p$.
%     \item $v_H(X)$ denote the vanishing polynomial over the multiplicative subgroup
% set $H$ defined by $\Pi_{i=0}^{i=n-1}(X- \omega^i)$ = $X^n -1$. Note that $v_H(\omega^i) = 0 \forall i \in \mathbb{N}$. 
%     \item $\ell_i(X)$ be $\Pi_{j \neq i} \frac{X - \omega^{j}}{\omega{i} - \omega^j}$ be $ith$ Lagarange polynomial that is unique and has degree $n-1$ such that $\ell_i(\omega^i) = 1$ and for $\ell_i(\omega^j) = 0$ for $j \neq i$.
% \end{itemize}
% Clearly, we can evaluate the interpolated polynomial by viewing the $a_i$ as evaluations of the polynomials.  another popular choice for independent polynomials in polycommit scheme is $1, X, X^2, \ldots, X^{n-1}$. 
% $$L_{\textbf{a}}(X) = \Sigma_{i =1}^n a_i\ell_i(X)$$

% Next we define our additional operations for committing evaluations(shares) of polynomials. Consider a well defined polycommit scheme $(\mathsf{PC.setup}$, $\mathsf{PC.commit}$, $\mathsf{PC.verifyeval}$, $\mathsf{PC.open}$, $\mathsf{PC.createwitness})$. We add a method to commit evaluations and combine evaluations. 
% \begin{itemize}
%     \item $\mathsf{PC.commitshare}(\mathsf{ck}, i, \share{x}, r)$ $\rightarrow$ $C_{\share{x}_i}$: 
%     Output a commitment to the evaluation at $\omega^i$ as  $\mathsf{PC.commit}(\mathsf{ck}, \share{x}*\ell_i(X), r)$. i.e
%     $g^{\share{x}*\ell_i(X)}h^r$ for $\mathsf{Polycommit_{Ped}}$.
%     \item $\mathsf{PC.combinecommitshares}(\mathsf{ck}, [C_{\share{x}_i}]_{i=0}^{n-1}) \rightarrow C_p$: 
%     Multiply the commitments to the homomorphically to obtain a commitment to the polynomial. Multiplication creates the $g^{p(X)} = g^{p_{\textbf{a}}(X)} = g^{\Sigma_{i =1}^n a_i\ell_i(X)}$.
% \end{itemize}


% The output commitment from the from $\mathsf{PC.combinecommitshares}$ is a polynomial commitment with the standard CRS $g, g^\beta, g^{\beta^2, \ldots}$ which we use evaluation proofs. In \ref{sec:server_compute} we show to create polycommit evaluation proofs for such commitments. We note that $g^{\ell_{i}(X)}$ can be pre-computed and hence the cost of commitment just one exponentiation and not $n$ exponentiation as would normally be required for committing a polynomial of degree $n$. 
% It is clear to see that if the underlying polycommit scheme is extractable, the above construction would also be extractable. 

\subsection{MPC protocol adaptations:}

\begin{figure*}[!htbp] 
\begin{boxedminipage}[t]{1\textwidth}
  {\centering \textbf{Robust Interpolation in the exponent}\\}

\textbf{Input:} Secret shared values $\share{x_i}$ from each server $P_i$.

\textbf{Output:} Pederson Commitment to $x$ of the form $g^xh^r$.

\textbf{Guarantees:} If $t< n/3$, then servers don't learn anything from $x$. 


For each MPC server $P_i$:


% \quad\emph{// Compute the function}
\begin{itemize}
    \item Use pre-processed random shares $\share{r_i}$ to compute share commitment  $C_{\share{x_i}} = g^{\share{x_i}}h^{\share{r_i}}$.
    \item Send commitment $C_{\share{x_i}}$ to all other servers $P_j$
    \item Use robust interpolation in the exponent to compute the commitment $g^xh^r$. In more detail, we note that all the Lagrange polynomials are fixed for the given set of $n$ parties. After receiving all the shares, we check easily the evaluate a candidate interpolation result polynomial $g^{p(x)}h^{p'(x)}$ at any point we desire. We can use that to check whether $2t + 1$ shares agree on some polynomial in the exponent. After finding such polynomial, we evaluate it at $0$ in the exponent and return $g^{f(0)}h^{r(0)}$ as $g^xh^r$
\end{itemize}
\end{boxedminipage}
\caption{Robust Interpolation in the exponent}
\label{fig:robust_exp_cli_input}
\end{figure*}


\begin{figure*}[!htbp] 
\begin{boxedminipage}[t]{1\textwidth}
  {\centering \textbf{MPC Polynomial Commitments from shares of evaluations}\\}

\textbf{Input:} Secret shared evaluations of a polynomial $\share{x_{i_1}}, \ldots, 
\share{x_{i_k}}$ from each server $P_i$.

\textbf{Output:} Hiding polynomial commitment $g^{p(X)}h^{r(X)}$ to polynomial $p(x)$ at degree at most $k-1$ which respects the evaluations $x_1, \ldots, x_k$.

\textbf{Guarantees:} If $t< n/3$, then servers don't learn anything from $p(X)$.

For each MPC server $P_i$:

% \quad\emph{// Compute the function}
\begin{itemize}
    \item Obtain a sharing of the polynomial $\share{p(X)}$ by locally interpolating at shares of evaluations $\share{x_{i_1}}, \ldots, \share{x_{i_k}}$. Use pre-processed random shares $\share{r_{i_1}}, \ldots, \share{r_{i_k}}$ to construct shares of hiding polynomial $\share{r(X)}$
    \item Compute $C_{\share{p(X)}} = \texttt{PC.commit(ck, \share{p(X)}, \share{r(X)})}$ and send the commitment $C_{\share{p(X)}}$ to all other parties.
    \item Use robust interpolation in the exponent to compute the commitment $g^{p(X)}h^{r(X)}$. The interpolation is carried out similarly to the method described in Figure \ref{fig:robust_exp_cli_input}
\end{itemize}
\end{boxedminipage}
\caption{MPC Polynomial Commitments from shares of evaluations}
\label{fig:mpc_polycommit}
\end{figure*}

\begin{figure*}[!htbp] 
\begin{boxedminipage}[t]{1\textwidth}
  {\centering \textbf{MPC Secret shared polynomials Create Witness}\\}

\textbf{Input:} Secret shared polynomials: Secret shares of evaluations of a polynomial $\share{x_{i_1}}, \ldots, \share{x_{i_k}}$ from each server $P_i$ and a evaluation point $\beta$. 

\textbf{Output:} Let $p(X)$ be the interpolated polynomial interpolated from the by combining the shares of the evaluations. The output consists of $(\pi, p(\beta))$ where $\pi$ = \texttt{PC.createwitness(p(X), $\beta$)}.

\textbf{Guarantees:} If $t< n/3$, then servers don't learn anything from $p(X)$ apart from $p(\beta)$

For each MPC server $P_i$:

% \quad\emph{// Compute the function}
\begin{itemize}
    \item Obtain a sharing of the polynomial $\share{p(X)}$ by locally interpolating at shares of evaluations $\share{x_{i_1}}, \ldots, \share{x_{i_k}}$. Use same hiding polynomial $\share{r(X)}$ which was used to creating the polycommit. 
    \item Compute $\share{\phi(X)} = \frac{\share{p(X)} - p(\beta)}{X - \beta}$, $\share{\hat{\phi}(X)} = \frac{\share{r(X)} - r(\beta)}{X - \beta}$ and send the commitment $C_{\share{\phi(X)}}$ = $g^{\share{\phi(X)}}h^{\share{\hat{\phi}(X)}}$  along with $\share{r(\beta)}$ to all other parties.
    \item Use robust interpolation in the exponent to compute the commitment $g^{\phi(X)}h^{r(X)}$ and $r(\beta)$. The interpolation is carried out similarly to the method described in \ref{fig:robust_exp_cli_input}
\end{itemize}
\end{boxedminipage}
\caption{MPC secret shared polynomials Create witness}
\label{fig:mpc_polycommit_createwitness}
\end{figure*}



\begin{figure*}[!htbp] 
\begin{boxedminipage}[t]{1\textwidth}
  {\centering \textbf{MPC Secret shared polynomials Evaluation}\\}

\textbf{Input:} Secret shared polynomials: Secret shares of evaluations of a polynomial $\share{x_{i_1}}, \ldots, \share{x_{i_k}}$ from each server $P_i$ and a evaluation point $\beta$. 

\textbf{Output:} Let $p(X)$ be the interpolated polynomial interpolated from the by combining the shares of the evaluations. The output consists of $p(\beta)$.

\textbf{Guarantees:} If $t< n/3$, then servers don't learn anything from $p(X)$ apart from $p(\beta)$

For each MPC server $P_i$:

% \quad\emph{// Compute the function}
\begin{itemize}
    \item Obtain a sharing of the polynomial $\share{p(X)}$ by locally interpolating at shares of evaluations $\share{x_{i_1}}, \ldots, \share{x_{i_k}}$. 
    \item Evaluate $\share{p(\beta)}$ and send it all other parties..
    \item Use regular Lagrange interpolation to obtain the value $p(\beta)$. 
\end{itemize}
\end{boxedminipage}
\caption{MPC secret shared polynomials evaluate}
\label{fig:mpc_poly_evaluate}
\end{figure*}


\begin{figure*}[!htbp] 
\begin{boxedminipage}[t]{1\textwidth}
  {\centering \textbf{Divmod operations on secret shared polynomials. }\\}

\textbf{Input:} Secret shared polynomials: Secret shares of evaluations of a polynomial $a(X)$ as  $(\share{x_{i_1}}, \ldots, \share{x_{i_k}})$, and another publicly known polynomial $b(X)$.

\textbf{Output:} Secret shared evaluations of resultant polynomial $r(X)$ after the corresponding
arithmetic operation $\share{q(X)}, \share{r(X)} = \share{a(X)}/b(X)$ such that $q(X)b(X) + r(X) = a(X)$
and degree($r(X)$) < degree($b(X)$).

\textbf{Guarantees:} If $t< n/3$, then servers don't learn anything from $a(X), b(X), r(X)$

For each MPC server $P_i$:

% \quad\emph{// Compute the function}
\begin{itemize}
    \item Obtain a sharing of the polynomial $\share{a(X)}$ by locally interpolating at shares of evaluations $\share{x_{i_1}}, \ldots, \share{x_{i_k}}$. 
    \item Use FFT based divmod on local shares of polynomials $\share{a(X)}$ to compute the shares of $\share{q(X)}, \share{r(X)}$. Appendix \ref{app:fft} shows the details of the polynomial division operation that can be our in $n\log{n}$
\end{itemize}
\end{boxedminipage}
\caption{Secret shared polynomial division with remainder by a publicly known polynomial}
\label{fig:mpc_divmod_local}
\end{figure*}


==> proofs_analysis/analysis.tex <==
\chapter{Analysis and Security Proofs:}
\section{Detailed protocol Analysis:}

%---------------------------------------------------------------------
\begin{table}[ht!]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ c c|c c|c c |c  }
\hline
& & \multicolumn{2}{|c|}{size/cost(bytes)} & \multicolumn{2}{c|}{Time Complexity}\\
\hline
  & & Comm & $|\pi|$ &  Prover & Auditor & Setup\\
 \hline
 \multirow{3}{1cm}{Vee'17} & $\mathbb{G}_1$ & - & 3$|X|$ + 8 & $\bigO{(n)}$ & 6$|X|$ + 12 pair. & \textsf{circ}  \\
                                     & $\mathbb{G}_2$ & - & - & - & - \\
                                     & $\mathbb{F}_q$ & - & - & $\bigO(m + n\log n)$ &- &  \\
\hline
 \multirow{3}{1cm}{This work} & $\mathbb{G}_1$ & $N(N-1)(|X| + 12)$ & 13 + $|X|$ & 21 v-MSM($3m$) + 7 v-MSM($N$) &  1 v-MSM$(|X|) + 2$ & \textsf{univ}  \\
                                     & $\mathbb{G}_2$ & - & - & - & 3(2*) pairings\\
                                     & $\mathbb{F}_q$ & $14N(N-1)$ & $23$ & $\bigO(N + m\log m)$ & $\bigO(\log m)$  \\
 \hline
%  Afghanistan	& AF	&AFG&	004\\
%  Aland Islands&	AX	& ALA	&248\\
%  Albania	&AL	& ALB&	008\\
%  Algeria	&DZ	& DZA&	012\\
%  American Samoa&	AS	& ASM&016\\
%  Andorra&	AD	& AND	&020\\
%  Angola&	AO	& AGO&024\\
%   \hline
 \end{tabular}
 }
 \begin{center}
 \caption{$M, N, m, n$ represents the maximum size of circuit, number of MPC parties, total number of gates and number of
 multiplication gates respectively. Comm, $\pi$ represent the total communication cost across all MPC servers and proof size.v-MSM($m$) denote variable-base multi-scalar multiplications (MSM) each of size $m$. It is possible to reduce the pairings to 2 pairings, however our implementation currently does not support it.}    
 \end{center}
 \label{table:complexity}
 \end{table}
%--------------------------------------------------------------------


We next show detailed analysis of our protocol in terms of exact number of group elements in ($\mathbb{G}_1$ and $\mathbb{G}_2$) and field elements($\mathbb{F}_q$). Note that Vee'17 does not report a detailed breakdown of proof elements so we use the $\bigO()$ asymptotic as shown in the paper. We note that despite our setup being universal, our proof size and auditor size are smaller than those of Vee'17 construction. 

This is because of different approaches to construction where the Vee'17 construction incurs penalty because of having to check pairings for each statement element. Although, Vee'17 prover does not show the exact prover computation numbers, we believe that the prover they have will be faster than ours because of access to circuit specific encoding in the exponent. This is to be expected as Marlin Prover\cite{chiesa2019marlin} is about 3-4 times slower than Groth16\cite{groth2016size}, which is state of the art circuit specific snark. We believe that if one can apply our ideas to Groth'16 SNARK, it possible to overcome these limitations. We leave exploring that as a future work as we were interested in diverse applicability Universal Setup.

Table \ref{table:complexity} shows the detailed comparison of our work with the previous work by Veeningen\cite{veeningen2017pinocchio}. Adaptive Trinochio construction in Vee'17 had a auditor do pairings 
of the order of statement size $|X|$ whereas our construction only uses 3 parings. Note that, it is possible to use an optimization detailed in Section 9 of Marlin\cite{chiesa2019marlin} to reduce this cost to 2 pairings. However, our implementation does not currently support this and hence we report our cost as 3 pairings instead of 2.

\begin{table}[ht!]
\begin{center}
 \begin{tabular}{||c| c| c c c||} 
 \hline
 - & Message Type & $\mathbb{G}_1$ & $\mathbb{G}_2$ & $\mathbb{F}_q$ \\ [0.5ex] 
 \hline\hline
 Initial Round & commitments & $|X|(N-1)$ & - & - \\ 
 \hline
 First Round & commitments & $4(N-1)$ & - & - \\
 \hline
 \multirow{3}{1cm}{Second Round} & commitments &$4(N-1)$ & - & - \\
                                & PolyEval proofs &$6(N-1)$ & - & $6(N-1)$ \\
                                & evaluations & - & - & $8(N-1)$ \\
 \hline
\end{tabular}
\end{center}
 \begin{center}
 \caption{Communication Cost breakdown per server  per round. $N$ represents the number of MPC servers and $|X|$ is the statement size. \label{table:round_analysis}}
 \end{center}
 \end{table}

Table \ref{table:round_analysis} shows the detailed round wise communication cost analysis for each round. In the initial round, the servers simply exchange the commitments to shares of statements, hence the per server cost is $|X|$. In the first round, the servers commit to the secret shared polynomials $w, mask, z_a, z_b$. The second round of communication consists of 3 separate messages sent together: 1) Commitments to $g_1$ and $h_1$, 2) evaluation proofs for $g_1, h_1, w, mask, z_a, z_b$ at $\beta_1$ and 3) evaluations of $x$ and $r$ polynomials. 

\input{analysis/proofs}

==> proofs_analysis/proofs.tex <==
\section{Proofs:}

In this section, we will show that completeness, extraction and zero-knowledge properties of our adaptive zk-snarks described in section \ref{fig:adapt-snark}. We show the following proofs assuming a Extractable $\textsf{PEC}$ scheme.


\begin{itemize}
    \item Perfect Completeness:
    
\textbf{Proof}: By inspection
\end{itemize}
\begin{itemize}
    \item Extractable: We say that our Snark is extractable if for every size bound $\mathsf{N} \in \mathbbm{N}$ and efficient adversary $\Adv$ = $(\Adv_1, \Adv_2)$ there exists an efficient extractor $\Ext$ such that
      \[
  \Pr \left[
    \begin{gathered}
    % \begin{gather}
    (\mathbf{C_x, \mathbbm{i, x, r, w})} \notin \mathcal{R}_{\mathsf{ck}_{eval}} \\
    \land \\
    \langle \mathsf{A_2}(\mathsf{st}) ,  \mathsf{V}(\mathsf{ivk}, \mathbf{C_x})\rangle = 1
    % \end{gather}
  \end{gathered}
    \middle|\\
        \begin{gathered}
    \mathsf{srs} \leftarrow \mathsf{G}(1^{\lambda}, \mathsf{N})\\
    \mathsf{ck_{eval}} \leftarrow \mathsf{PEC.Setup}\\
    (\mathbf{C_x, \mathbbm{i}, \mathsf{st})} \leftarrow \Adv_1(\mathsf{srs; z})\\
    (\mathbbm{x, r, w}) \leftarrow \Ext^{A_1}(\mathsf{srs; z}) \\
    \mathsf{ipk, ivk} \leftarrow \mathsf{I}^{\mathsf{srs}}(\mathbbm{i}) \\
    \end{gathered}
  \right] = \mathsf{negl}(\lambda)
  \]
\end{itemize}

The output proof from $\Adv_2$ would be of the form ($\mathsf{prf_{mar}, v, \pi_{comm}, \mathbf{C^{\mathbbm{b}}_x}}$).
We construct our extractor $\Ext$ as follows:
\begin{itemize}
    \item Use the Commitment Extractor $\Ext_{comm}$ to extract inputs and randomness $\mathbbm{x,r}$ from augment statement commitments $\mathbf{C_x}, \mathbf{C^{\mathbbm{b}}_x}$.
    \item Use the marlin extractor $\Ext_{Mar}$ with above extracted statement $\mathbbm{x}$ and $\mathsf{prf_{mar}}$ to get witness $\mathbbm{w}$. The constructions of this extractor is described in Section 8.3 of Marlin\cite{chiesa2019marlin} paper. 
    \item Use the same $\mathbbm{i}$ as the one output by the $\Adv_1$ and output $\mathbbm{(x, r, w, i)}$
\end{itemize}

We need to show that, if $\Adv$ = $(\Adv_1, \Adv_2)$  produces a verifying proof, the extractor fails
only with negligible probability and the returned values are in $\mathcal{R}_{\mathsf{ck}_{eval}}$.

Suppose that $\Ext$ fails with non-negligible probability $\epsilon$, then either two extractors ($\Ext_{comm}$ or $\Ext_{Mar}$) fail or the output $\mathbbm{(x, r, w, i)} \notin \mathcal{R}_{\mathsf{ck}_{eval}}$

\begin{itemize}
    \item If $\Ext_{Mar}$ fails, then we can construct an adversary that makes the extractor fail to either break 1) the soundness of underlying Algebraic Holographic Proof(AHP) or 2) succeed in the extractability game for the PC scheme. We defer the reader to the Section 8.3 of Marlin paper\cite{chiesa2019marlin} for details.
    \item If the $\Ext_{comm}$ fails with non-negligible probability, then we can break the extraction game for the $\mathsf{PEC}$ scheme.
\end{itemize}

It remains to show that the values returned by the extractor are in with high probability in $\mathcal{R}$. Recall that: 
$$\mathcal{R}_{\mathsf{ck}_{eval}} := \{(\mathbf{C_x, \mathbbm{i}, \mathbbm{x}, r, \mathbbm{w})}) : \forall i \ C_{x_i} = \mathsf{PEC.Commit_{eval}}(\mathsf{ck_{eval_i}}, x_i, i, r_i) \land (\mathbbm{x},\mathbbm{i}, \mathbbm{w}) \in \mathcal{R}\}$$

By properties of the extractor $\Ext_{comm}$, we know that openings to the commitments $\mathbf{C_x}$ are ($\mathbbm{x, r}$) and now we need to show that $(\mathbbm{x},\mathbbm{i}, \mathbbm{w}) \in \mathcal{R}$. Let the interpolated polynomial for all $\mathbbm{x}$ be $\tilde{x}(X)$.

Note that in regular Marlin execution, the value $\mathsf{v}$ is computed the verifier himself based on the statement $x$. We need show that with high probability that the $\mathsf{v}$ is exactly the same of $\hat{x}(\beta_1)$. Suppose that this were not the same, $\mathsf{v} \neq \hat{x}(\beta_1)$. i.e $\tilde{x}(\beta_1) \neq \hat{x}(\beta_1)$ which means that $\hat{x}(X) \neq \tilde{x}(X)$.

From the completeness of underlying AHP Marlin protocol, we know that 
$$\hat{z}(X) := \hat{w}(X)v_H(X) + \hat{x}(X)$$
is true for all the values of $X$. Therefore, the equation can only hold true for $\tilde{x}$ with probability $|X|/|\mathbbm{F}|$ for a randomly sampled challenge $\beta_1$ from the verifier. $|X|$ is the statement length and also the degree of the polynomial $\hat{x}$.

\begin{itemize}
    \item Zero Knowledge: We say that our Snark is zero knowledge if there exists a simulator $\mathsf{S = (S.Setup, S.Prove)}$ if for every efficient adversary $\Adv$ = $(\Adv_1, \Adv_2)$ it holds that
      \[
  \Pr \left[
    \begin{gathered}
    % \begin{gather}
    (\mathbf{C_x, \mathbbm{i, x, r, w})} \in \mathcal{R}_{\mathsf{ck}_{eval}} \\
    \land \\
    \langle \mathsf{P}(\mathsf{ipk}, \mathsf{ck_{eval}}, \mathbf{C_{x}}, \mathbf{x}, \mathbf{r}, \mathbf{w}) ,  \mathsf{\Adv_2}(\mathsf{st})\rangle = 1
    % \end{gather}
  \end{gathered}
    \middle|\\
        \begin{gathered}
    \mathsf{srs} \leftarrow \mathsf{G}(\mathsf{N})\\
    \mathsf{ck_{eval}} \leftarrow \mathsf{PEC.Setup}\\
    (\mathbf{C_x, \mathbbm{i, x, r, w)}, \mathsf{st})} \leftarrow \Adv_1(\mathsf{srs})\\
    \mathsf{ipk, ivk} \leftarrow \mathsf{I}^{\mathsf{srs}}(\mathbbm{i}) \\
    \end{gathered}
  \right] = 
  \]
    \[
  \Pr \left[
    \begin{gathered}
    % \begin{gather}
    (\mathbf{C_x, \mathbbm{i, x, r, w})} \in \mathcal{R}_{\mathsf{ck}_{eval}} \\
    \land \\
    \langle \mathsf{S.Prove}(\mathsf{td_{srs}}, \mathsf{td_{comm}}, \mathbf{C_{x}}, \mathbbm{i}) ,  \mathsf{\Adv_2}(\mathsf{st})\rangle = 1
    % \end{gather}
  \end{gathered}
    \middle|\\
        \begin{gathered}
    \mathsf{srs, td_{comm}, td_{srs}} \leftarrow \mathsf{S.Setup}(\mathsf{N})\\
    (\mathbf{C_x, \mathbbm{i, x, r, w)}, \mathsf{st})} \leftarrow \Adv_1(\mathsf{srs})\\
    \end{gathered}
  \right]
  \]
\end{itemize}

We need to the simulator with access to the trapdoor can generate proofs that can indistinguishable from real proofs. In other words, our simulator $\mathsf{S}$ is given given commitments to the $\mathsf{C_x}$ and needs to construct proofs using the trapdoors from commitment scheme and trapdoor from marlin. Our simulator works as follows: 


\begin{figure*}[!htbp] 
\begin{boxedminipage}[t]{1\textwidth}
  {\centering \textbf{Simulator for Adaptive ZK Consturction in \ref{fig:adapt-snark} }\\}

\begin{itemize}
    \item Recall that our proof consists of four elements ($\mathsf{prf_{mar}, v, \pi_{comm}, \mathbf{C^{\mathbbm{b}}_x}}$). First, the simulator samples a random polynomial $\hat{x}$ of
    $\mathsf{deg(|C_x|)} + \mathsf{deg}(|C^{\mathbbm{b}}_x|)$. 
    Note that all the information simulator needs is the length of the augmented statement.
    \item Using the trapdoors of the $\mathsf{PEC}$, open the commitments $\mathbf{C_x}$ to corresponding evaluations of $\hat{x'}$ over a pre-selected domain. Extend the polynomial by degree $\mathbbm{b}$ to get a resultant polynomial $\hat{x}$. Create a commitment to the additainal $\mathbbm{b} $evaluations as $(|C'^{\mathbbm{b}}_x|)$.
    \item Run the marlin simulator with $\hat{x}$ to obtain a fake proof $\mathsf{prf'_{mar}}$ and obtain the evaluation $\hat{x}(\beta_1)$.
    \item Interpolate the commitments $\mathbf{C_x}$ using $\mathsf{PEC.interpolate}$ to obtain a polynomial commitment $c_p$ for the $\hat{x}$ and provide a evaluation proof $\mathsf{\pi'_{comm}}$ for the correct value $\hat{x}(\beta_1)$.
    \item return the proof ($\mathsf{prf'_{mar}},
    \hat{x}(\beta_1)$ 
    $\mathsf{\pi'_{comm}}$, $(|C'^{\mathbbm{b}}_x|)$).
\end{itemize}

\end{boxedminipage}
\caption{Simulator construction for adaptive zk-snark}
\label{fig:sim_adapt_zk}
\end{figure*}
The figure \ref{fig:sim_adapt_zk} shows the construction for simulator satisfying the above definition for our construction in \ref{fig:adapt-snark}. Next, we provide a proof about the indistinguishably for the ideal and real world for the adversary w.r.t our simulator.

First, we note that in the underlying AHP for $x$ polynomial, we also have introduced a query bound $\mathbbm{b}$ in order to ensure zero knowledge of the evaluations of $x$ upto $\mathbbm{b}$ queries.
Informally, since the prover sampled $\hat{x}$ such that $\mathsf{deg(\hat{x}) = deg(x) + \mathbbm{b}}$ queries less than the query bound $\mathbbm{b}$ information theoretically does not reveal any information about $x$.

Similar to the construction in \cite{ben2019aurora},  we would construct a simulator $\mathsf{AHP'}$ for the underlying AHP with changes that the first message of the prover also includes an
encoding of statement along with the encoding of witness and encoding of its linear combinations. These encodings are protected against up to $\mathbbm{b}$ queries because the encodings have degree $\mathbbm{b} $more than than corresponding encodings. The rest of simulator for the subsequent rounds proceeds similar to what is described in Marlin\cite{chiesa2019marlin}. At the high level, all the subsequent messages are hidden by adding the additional $\mathsf{s}$ polynomial and hence do not reveal any information. 

From the marlin simulator with the trapdoors to $\mathsf{srs}$ which uses $\mathsf{AHP'}$ instead of
$\mathsf{AHP}$ described in marlin, we know that $\mathsf{prf'_{mar}}$ and $\mathsf{prf_{mar}}$ are
indistinguishable. For the last proof element 
$\mathbf{C'^{\mathbbm{b}}_x}$ is indistinguishable from $\mathbf{C^{\mathbbm{b}}_x}$. 
Similarly, using the trapdoors $\mathsf{td_{comm}}$ for $\mathsf{PEC}$, we can simulated proofs for $(\pi'_{comm},
\hat{x}(\beta_1))$ are indistinguishable from $(\mathsf{\pi_{comm}, v})$. 

Although, we have argued about the individual distributions of $\mathsf{prf'_{mar}}$ and $\mathsf{prf_{mar}}$ are same and distributions for $(\mathsf{\pi_{comm}, v, }, $ and $(\pi'_{comm}, \hat{x}(\beta_1))$. Similarly, we also showed that $\mathbf{C'^{\mathbbm{b}}_x}$ is indistinguishable from $\mathbf{C^{\mathbbm{b}}_x}$. We observe that calculation of the proof elements for $\mathsf{prf'_{mar}}$ is independent of the choices made by the simulator in $\pi'_{comm}$ experiment. Thus, we can argue that the joint distributions are identically distributed. 

==> related_work/related_work.tex <==
\section{Related Work}
\sanket{Trim this down}
Zk-SNARKs (Zero-knowledge Succinct Non-Interactive Arguments of Knowledge) have risen as a popular solution for fast verification of arithmetic relations. Over the past decade, several zk-SNARKs like Pinocchio~\cite{parno2013pinocchio}, Groth's constructions~\cite{groth2010short}~\cite{groth2008efficient}~\cite{groth2016size} and many others have made pairing based zk-SNARKs practical. Most of these pairing approaches required circuit-specific common reference string ($\mathsf{srs}$), which requires a trusted third party to generate \textit{toxic waste} (intermediate computations that must be destroyed after setup). On the other hand, approaches like bulletproofs~\cite{bunz2018bulletproofs}, STARKs~\cite{ben2014succinct,ben2016quasi,ben2017interactive,ben2017scalable,ben2019scalable,ben2019aurora}, hyrax~\cite{wahby2018doubly} and ZKboo~\cite{giacomelli2016zkboo,chase2017post} rely on uniform random strings ($\mathsf{urs}$), which do not have such toxic waste but suffer from practical performance drawbacks in verification time. As a compromise between these approaches, a one-time universal setup~\cite{groth2018updatable,maller2019sonic,setty2019spartan,gabizon2019plonk,chiesa2019marlin} has emerged as a popular alternative to achieve the efficiency of pairing-based approaches with minimal only one-time toxic waste that is not circuit specific. We base our construction on a state of the art universal updatable zk-SNARK Marlin~\cite{chiesa2019marlin} and show how to adapt the zk-SNARK proof generation via MPC. 
%LegoSnark~\cite{campanelli2019legosnark} show how to compose different ``Commit and Prove" (CaP) SNARKs from different gadgets.

Auditable protocols have been studied extensively in, for example, electronic voting applications and secret sharing applications. Public verifiability was introduced by Cohen and Fischer in 1985~\cite{cohen1985robust}. Helios~\cite{adida2008helios}, the first web-based open audit voting system, is perhaps the best known example. A majority of research in auditing protocols has focused on specific applications like elections~\cite{schoenmakers1999simple,kusters2010accountability,sako1995receipt,moran2006receipt}, auctions~\cite{naor1999privacy,sako2000auction} or secret shared dealing~\cite{schoenmakers1999simple,fujisaki1998practical,stadler1996publicly}. In a recent work, Chen et al.~\cite{chendiogenes} propose a strong notion of security with identifiable-abort along with public-auditability for generating an RSA modulus.

The notion of public auditable MPC for general arbitrary computations was first introduced by Baum et al.~\cite{baum2014publicly}. The authors base their work on SPDZ~\cite{damgaard2012multiparty,damgaard2013practical}. However, Baum's protocol has the auditor look at the entire protocol transcript, and hence the audit phase has verification time and proof size linear in the size of the computation. In a client-server MPCSaaS model, where lightweight clients want to audit the protocol execution, a linear audit is prohibitively expensive.  Trinocchio~\cite{schoenmakers2016trinocchio} protocol offers a multi-party based construction for Pinocchio proof generation. 

Veeningen showed~\cite{veeningen2017pinocchio} how to make the Trinocchio protocol adaptive (computations are chosen after the input data is committed), which closely resembles our work. The construction from Veeningen~\cite{veeningen2017pinocchio} relies on a circuit-specific setup and invoking a trusted third party for new circuit computation, whereas our construction has no such drawback. Secondly, Veeningen's construction only considers a single-shot execution of MPC because of which it faces no communication cost for MPC computation. In order to avoid the extra communication, they outsource the combination of proofs to the auditor, which makes the total proof size proportional to the number of servers. Our construction supports reactive MPC style computations (using outputs of previous rounds as inputs to new MPC rounds), and our proof size does not increase with the number of MPC servers but instead incurs three rounds of communication overhead. Third, in order to achieve input independence (parties cannot choose their input on inputs of other parties), Veeningen's construction introduced a keyed-commitment scheme even when all MPC servers are corrupt. We show that it is not possible to achieve input independence when all servers are corrupt in a reactive MPC and therefore base our construction on a simpler commitment scheme. For single-shot MPC, we also show how to extend our construction to achieve input independence for single-shot MPC using a new commitment scheme. Finally, because of statement embedding the proof checking, the auditor in Veeningen's construction has pairing cost linear in the number of commitments while we only incur a penalty in group operations(far cheaper than pairings) and keep constant pairing costs.

%Over the past two decades, lots of research by Schoenmakers et al.~\cite{schoenmakers1999simple}, K\"usters et al.~\cite{kusters2010accountability}, Sako et al.~\cite{sako1995receipt} and Moran et al.~\cite{moran2006receipt} have considered a publicly auditable election protocols. Recently, Chen et al.~\cite{chendiogenes} also propose a public auditable RSA modulus construction that can support thousands of parties and offers security against an arbitrary number of corrupted parties. Even among the few known useful applications of MPC already in deployment, such as RSA modulas construction it's already important that they satisfy public auditability. When this has been provided, it's for a custom protocol.  
%So far, none of the implementations of generic MPC frameworks have provided this feature. 
\ignore{
\textbf{Fast auditor with one-time universal setup:} 
In the MPCSaaS setting, typically low-powered clients sending outsourcing computation to the high-power servers. Thus, in order to audit the computation, the computation proof size must be small, and proof verification must be fast. Fast auditing is crucial in applications like secure election and cryptocurrency parameter generation, where the computation proofs are to be checked by a large number of low powered participants. Previous work by Baum et al.~\cite{baum2014publicly} gave the first construction for auditable MPC; however, it involved the auditor reading the entire transcript, which would be inefficient for many practical applications. 

Snarks have gained popularity as a for fast enable verifying NP statements. Over the years, numerous constructions~\cite{maller2019sonic}~\cite{chiesa2019marlin}~\cite{bunz2018bulletproofs}~\cite{wahby2018doubly}~\cite{zhangtransparent}~\cite{bunz2019transparent} of ZK-snarks have been proposed improving efficiency, proof size and verification times. In almost all of the constructions, proofs are verified with respect to plaintext inputs of the verifier; but for our reactive auditable(Refer section ~\ref{sec:prelim_reactive_mpc}) MPC application,  we want such proofs
to able to be adaptive, meaning computations can be chosen after the input data has been committed. 

Amongst the adaptive SNARKs, the hash-first approach suggested by Fiore et al.~\cite{fiore2016hash} for adaptive verifiable computations on outsourced data is not zero-knowledge. The construction by Lipmaa~\cite{lipmaa2017prover} for CaP SNARKs is zero knowledge but relies on a subset-sum language instead of R1CS language. In more detail, even tough the Subset-Sum and R1CS languages are both NP-complete, most MPC computations are more naturally expressed as R1CS constraints whereas expressing the same in Subset Sum language would incur practical concrete overhead. 
Finally, another construction by Veeningen~\cite{veeningen2017pinocchio} shows how to adapt Trinocchio~\cite{schoenmakers2016trinocchio} for secure function evaluation. It, however, relies on a trusted third party to compute a circuit-specific setup for every new unknown computation. Generating a trusted setup server as a practical problem as to how to instantiate this party. The servers cannot be trusted to create this setup as our trust model involves all malicious servers. A one-setup can include the setups for some known circuits, but such a scenario one cannot change the computation after the setup. For deployment of auditable MPCSaaS, providers cannot know what computations the clients will be performing. Even if the client computations are known beforehand, clients can, at a later time, can request to update the computation because of implementation bugs or performance improvements. For a circuit-specific setup, it is not possible to update the computation without invoking a trusted third party. 

Our construction is based on Marlin~\cite{chiesa2019marlin} instead of Pinocchio~\cite{parno2013pinocchio} and thus does not require a trusted party for such a computation. For the same reason it is also updateable~\cite{groth2018updatable}, which means that it can be rerandomized by new parties as well, refreshing its security (soundness only relies on any one out of all the parties who have updated it). 
}

% The original 
% Comparison to Vee'17:
% \begin{itemize}
%     \item Universal vs circuit trusted setup: Vee'17 requires calling the trusted party for each invocation for a new secure computation. 
%     \item Commitments (keyed commitment vs pederson commitments)
%     \item Input independence and input robustness 
%     \item non-robust semi-honest MPC single-shot setting vs reactive setting. Does not use pre-processing in MPC for optimizations or robustness. 
%     \item Does not have auditable MPC, but targets more secure computation.  
% \end{itemize}

% Comparison to Baum'14:
% \begin{itemize}
%     \item Introduces the concept of auditable MPC. This does actually define the auditor and the first formal notion of auditable MPC, but is not succinct. The auditor looks at entire transcript
%     \item They also address auditing the offline phase, which is out of the scope of our current work. Kindof a negative point, maybe not worth explicitly writing. 
%     \item Does not address robust setting of MPC computation and only gives a solution in semi-honest case.
%     \item Only a theoretical introduction with no practical implementation benchmarks. 
% \end{itemize}


